Controllable Data Augmentation for Few-Shot Text Mining with Chain-of-Thought Attribute Manipulation

Prompting large language models (LLMs) for data augmentation has recently become a common practice in few-shot NLP tasks. In this paper, we propose Chain-of-Thought Attribute Manipulation (CoTAM), a novel approach that generates new data from existing examples by only tweaking in the user-provided, task-specific attribute, e.g., sentiment polarity or topic in movie reviews. Instead of conventional latent representation controlling, we leverage the chain-of-thought prompting to directly edit the text in three steps, (1) attribute decomposition, (2) manipulation proposal, and (3) sentence reconstruction. Extensive results on various tasks, such as text (pair) classification, aspect-based sentiment analysis, and conditional text generation, verify the superiority of CoTAM over other LLM-based augmentation methods with the same number of training examples for both fine-tuning and in-context learning. Remarkably, the 2D visualization of the augmented dataset using principal component analysis revealed a human-recognizable decision boundary that is likely hinted by the attribute manipulation, demonstrating the potential of our proposed approach.

==> rebuttal-r2.tex <==
% % This must be in the first 5 lines to tell arXiv to use pdfLaTeX, which is strongly recommended.
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Remove the "review" option to generate the final version.
% \usepackage[review]{ACL2023}
% % \usepackage{ACL2023}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}

% \usepackage{bbding}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{arydshln}
% \usepackage{bbm}
% \usepackage{booktabs}
% \usepackage{CJKutf8}
% \usepackage{combelow}
% \usepackage{enumitem}
% \usepackage{epsfig}
% \usepackage{fancybox}
% \usepackage{float}
% \usepackage{graphicx}
% \usepackage{hyperref}
% \usepackage{multirow}
% \usepackage{multicol}
% \usepackage{pgfplots}
% \usepackage{pifont}
% \usepackage{setspace}
% \usepackage{subfigure}
% \usepackage{tabularx}
% \usepackage{url}
% \usepackage{xspace}
% \usepackage[vlined,ruled,commentsnumbered,linesnumbered]{algorithm2e}

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % This is not strictly necessary, and may be commented out.
% % However, it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}
% \usepackage{enumitem}

% % This is also not strictly necessary, and may be commented out.
% % However, it will improve the aesthetics of text in
% % the typewriter font.
% \usepackage{inconsolata}

% \newcommand{\jingbo}[1]{\textcolor{blue}{\bf\small [#1 -- JS]}}
% \newcommand{\letian}[1]{\textcolor{red}{\bf\small [#1 -- LT]}}
% \newcommand{\yuwei}[1]{\textcolor{orange}{\bf\small [#1 -- YZ]}}

% \newcommand{\dep}[1]{\textcolor{red}{\bf\small [Dependency Required: #1]}}

% \newcommand{\ready}[0]{\textcolor{blue}{\bf\small [Ready for Writing]}}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% % \title{Generating Efficient Few-shots via LLM-based Attribute Manipulation}
% % \title{Chain-of-Thought Attribute Manipulation for Few-shot Data Augmentation}
% \title{Controllable Data Augmentation for Few-Shot Text Mining with\\ Chain-of-Thought Attribute Manipulation}

% \author{Letian Peng \and Yuwei Zhang \and Jingbo Shang\thanks{$\ $  Corresponding author. } \\
% University of California, San Diego \\
%   \texttt{\{lepeng, yuz163, jshang\}@ucsd.edu}
%   }

% % New commands
% \newcommand{\method}{CoTAM\xspace}
% \newcommand{\smallsection}[1]{\noindent\textbf{#1}.}
% \newcommand{\fullmethod}{Chain-of-Thought Attribute Manipulation\xspace}

% \begin{document}
% % \maketitle

% \section{Update}

% We appreciate the effort of all reviewers to improve the quality of our paper. We have multiple updates on the previous version and hope these updates will meet your expectation of our work!

% \subsection{Experiments on Open-sourced LLMs}

% \begin{table}[H]
% \centering
% \small
% \scalebox{0.8}{\begin{tabular}{llccccccc}
% \toprule
% \multicolumn{2}{l}{\textbf{Method}} & SST-2 & TweetEmo & AG-NEWS \\
% \midrule
% \multirow{6}*{\rotatebox{90}{Fine-tuning}} & Base & $60.54$ & $44.38$ & $81.05$ \\
% & Extra Annotation$^\dag$ & $62.17$ & $69.51$ & $88.66$ \\
% & LLM Pseudo Label & $61.37$ & $66.85$ & $78.51$ \\
% & FlipDA++ & $73.91$ & $66.94$ & $82.56$ \\
% & CoTDA & $71.77$ & $63.46$ & $83.03$ \\
% & \method & $\textbf{74.83}$ & $\textbf{67.97}$ & $\textbf{83.49}$ \\
% \midrule
% \multirow{6}*{\rotatebox{90}{ICL}} & Base & $88.40$ & $65.20$ & $44.00$ \\
% & Extra Annotation$^\dag$ & $88.90$ & $77.80$ & $76.20$ \\
% & LLM Pseudo Label & $88.60$ & $\textbf{74.20}$ & $56.90$ \\
% & FlipDA++ & $\textbf{89.90}$ & $71.80$ & $68.30$ \\
% & CoTDA & $88.70$ & $69.90$ & $73.90$ \\
% & \method & $\textbf{89.90}$ & $72.80$ & $\textbf{75.30}$\\
% \bottomrule
% \end{tabular}}
% \caption{Repeated experiments of the main experiments with open-sourced LLM (\texttt{llama-2-70b-chat-hf}), which is applied to both data generation and in-context learning.}
% \label{tab:main-open}
% \end{table}

% To improve the reproducibility of our results, we present results on open-sourced LLMs as presented in Table~\ref{tab:main-open}. We present the fine-tuning and ICL results on three datasets here and have more results in the new version of the paper. The performance of different augmentation methods on the open-sourced LLM is generally consistent with our main experiments.

% \subsection{Conditional Text Generation}

% \begin{table}[H]
% \centering
% \small
% \scalebox{0.95}{
% \begin{tabular}{lcccccc}
% \toprule
% \multirow{2}*{\textbf{Method}} & \multicolumn{4}{c}{CommonGen} \\
% \cmidrule(l){2-5}
%  & Rouge-1 & Rouge-2 & Rouge-L & Coverage \\
% \midrule
% Base & $41.99$ & $13.98$ & $33.57$ & $65.07$ \\
% Extra$^\dag$ & $46.30$ & $15.66$ & $36.18$ & $75.55$ \\
% LLM SL & $\textbf{47.85}$ & $14.68$ & $35.63$ & $75.95$ \\
% FlipDA++ & $46.81$ & $14.48$ & $35.32$ & $\textbf{76.10}$ \\
% CoTDA & $44.43$ & $13.43$ & $35.05$ & $65.98$ \\
% CoTAM & $46.38$ & $\textbf{15.85}$ & $\textbf{37.02}$ & $75.23$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{The performance of span manipulation on conditional text generation. \textbf{Coverage} means the ratio of given keywords that appeared in the output sentence.}
% \label{tab:commongen}
% \end{table}

% We run experiments on the CommonGen dataset to apply our \method to conditional text generation. CommonGen targets to generate a sentence that contains a set of keywords. For instance, with input words: ``ski, mountain, skier'', the output can be ``Skier skis down the mountain'' We use CoTAM to manipulate the data by switching the group of keywords to another one (proposed by the LLM) while keeping other attributes unchanged.

% According to the metrics shown in Table~\ref{tab:commongen}, we can view CoTAM holds its advantage over other LLM-based augmentation methods. Thus, we conclude that CoTAM is not only limited to classification tasks but also has the potential for information extraction and natural language generation.

% \subsection{Clustering Analysis}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.49\textwidth]{figures/attribute_pca.pdf}
% \caption{The statistics the most frequent $10$ attributes in the decomposition step of \method.}
% \label{fig:attribute_pca}
% \end{figure} 

% We also present a new analysis of the semantic distribution of the attributes. We use the sentence encoder to encode the attribute names and run K-Means ($K=10$) clustering, which is presented in Figure~\ref{fig:attribute_pca}. We find the attributes that are the closest to the cluster centers and get $10$ attributes: 

% \begin{itemize}
%     \item an implied evaluation or opinion
%     \item a passive tone
%     \item subject (X)
%     \item subjectivity
%     \item action (X)
%     \item it mentions specific elements of a film (X)
%     \item brevity: short phrase
%     \item focus (X)
%     \item evocative
%     \item comparison (X)
% \end{itemize}

% \noindent which shows the diversity of the discovered attributes and improves our understanding of the attribute distribution in the pipeline.

% \subsection{Pipeline Case Study}

% We also incorporate a case study to compare different text manipulation pipelines to more specifically show the difference between different methods. 

% \section{Response to Meta Reviewer}

% Thank you for expressing concern about the reproducibility of our results. We repeat the whole main experiments on an open-sourced LLM (\texttt{llama-2-70b-chat-hf}) to improve the reproducibility of our results in the new version. 

% \section{Response to Reviewer Yiv4}

% We are thankful for your positive view of our work. We agree that the textual nature of our CoTAM pipeline will limit its application to attributes that cannot be expressed by text. However, with this limitation, our CoTAM can still be applied for tasks more than classification, such as aspect-based sentiment analysis and conditional text generation, as shown in the new version.

% \section{Response to Reviewer JVeE}

% We appreciate your support for the positive impact of our work. We have incorporated a variety of new results to improve the reproducibility, scope, and understanding of our CoTAM to further improve the quality of our work. 

% \section{Response to Reviewer CxLC}

% Thanks for your suggestion on incorporating a case study to compare different augmentation methods. We follow your suggestion to add the case study to more specifically illustrate the method differences.

% \end{document}

==> rebuttal.tex <==
% % This must be in the first 5 lines to tell arXiv to use pdfLaTeX, which is strongly recommended.
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Remove the "review" option to generate the final version.
% \usepackage[review]{ACL2023}
% % \usepackage{ACL2023}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}

% \usepackage{bbding}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{arydshln}
% \usepackage{bbm}
% \usepackage{booktabs}
% \usepackage{CJKutf8}
% \usepackage{combelow}
% \usepackage{enumitem}
% \usepackage{epsfig}
% \usepackage{fancybox}
% \usepackage{float}
% \usepackage{graphicx}
% \usepackage{hyperref}
% \usepackage{multirow}
% \usepackage{multicol}
% \usepackage{pgfplots}
% \usepackage{pifont}
% \usepackage{setspace}
% \usepackage{subfigure}
% \usepackage{tabularx}
% \usepackage{url}
% \usepackage{xspace}
% \usepackage[vlined,ruled,commentsnumbered,linesnumbered]{algorithm2e}

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % This is not strictly necessary, and may be commented out.
% % However, it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}
% \usepackage{enumitem}

% % This is also not strictly necessary, and may be commented out.
% % However, it will improve the aesthetics of text in
% % the typewriter font.
% \usepackage{inconsolata}

% \newcommand{\jingbo}[1]{\textcolor{blue}{\bf\small [#1 -- JS]}}
% \newcommand{\letian}[1]{\textcolor{red}{\bf\small [#1 -- LT]}}
% \newcommand{\yuwei}[1]{\textcolor{orange}{\bf\small [#1 -- YZ]}}

% \newcommand{\dep}[1]{\textcolor{red}{\bf\small [Dependency Required: #1]}}

% \newcommand{\ready}[0]{\textcolor{blue}{\bf\small [Ready for Writing]}}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% % \title{Generating Efficient Few-shots via LLM-based Attribute Manipulation}
% % \title{Chain-of-Thought Attribute Manipulation for Few-shot Data Augmentation}
% \title{Controllable Data Augmentation for Few-Shot Text Mining with\\ Chain-of-Thought Attribute Manipulation}

% \author{Letian Peng \and Yuwei Zhang \and Jingbo Shang\thanks{$\ $  Corresponding author. } \\
% University of California, San Diego \\
%   \texttt{\{lepeng, yuz163, jshang\}@ucsd.edu}
%   }

% % New commands
% \newcommand{\method}{CoTAM\xspace}
% \newcommand{\smallsection}[1]{\noindent\textbf{#1}.}
% \newcommand{\fullmethod}{Chain-of-Thought Attribute Manipulation\xspace}

% \begin{document}
% % \maketitle

% \section{Response to Reviewer Znfs}

% Thank you for your valuable suggestions, which have greatly enhanced our work. We have conducted additional experiments and analyses to address your concerns about the technical depth of our study.

% \paragraph{CoTAM Workflow Demonstration} In Section 5.1, we've included a diagram illustrating how CoTAM effectively manipulates text attributes. This visual aid demonstrates CoTAM's capability to capture and maintain the attributes of texts across various dimensions during reconstruction. For different input texts, CoTAM adeptly identifies and controls relevant attributes, aligning with our design objectives.

% \paragraph{More Complex Manipulation} We've extended CoTAM's application beyond simple classification. Our new experiments on Aspect-Based Sentiment Analysis showcase CoTAM's superiority over other LLM-based augmentation methods. The results from the SemEval14 dataset confirm CoTAM's effectiveness.

% \section{Response to Reviewer 3io3}

% We appreciate your positive feedback on our manuscript. Following your suggestions, we have thoroughly revised our writing. Section 3 has been restructured for better clarity, including improved demonstrations and method proposals. Also, we revise overview (Figure 2) to illustrate a more clear scenario of our manipulation. These revisions emphasize our core concept of manipulating the target attribute while preserving other irrelevant attributes. Additionally, we corrected the "CoTAG" typo to "CoTDA" in Section 5.2 of the new submission.

% \section{Response to Reviewer xEcb}

% Thank you for acknowledging the novelty of our work. Our study primarily demonstrates the potential of LLMs in manipulating text attributes purely through text, diverging from traditional image manipulation in latent space. In Section 5.3, we illustrate the consistency in manipulation directions within the latent space, which validates the effectiveness of in-context manipulation in CoTAM. We've also added a \textbf{CoTAM Workflow Demonstration} in Section 5.1 to better explain the dynamic decomposition process for attribute manipulation.

% \section{Response to Meta Reviewer}

% We are grateful for your comprehensive and insightful feedback, which has been instrumental in refining our work. Beyond its practical implications, our study enriches the understanding of LLMs by showcasing their capability in text attribute manipulation, especially in a pure text manner. Figure 5.3 demonstrates CoTAM's effective manipulation trajectory within the latent space of sentence embeddings, confirming the LLM's proficiency as a pure text manipulator. To further explore and enhance LLM utility, we've introduced the \textbf{Workflow of CoTAM} and incorporated ABSA experiments for \textbf{More Complex Manipulation}.

% \paragraph{In-context Learning} In Section 4, we delve into how CoTAM aids in-context learning (ICL) in LLMs. We compare the ICL performance of LLMs with various augmentation methods based on limited human annotations. Our findings confirm that CoTAM surpasses other methods, highlighting its broader application in few-shot learning, particularly when LLMs are accessible.

% We have also carefully restructured the sections and refined the figures in the new submission, ensuring clearer formalization and detailed preliminaries. We believe this revised version effectively addresses your concerns regarding the previous submission's shortcomings.

% \end{document}
